Data-Adaptive Mahalanobis Metric Learning for Cross-Head Attention in Transformers

In this paper, we propose Data-Adaptive Mahalanobis Cross-Head Attention (DAMCHA), a simple and effective attention mechanism that generalizes Multi-Head Attention (MHA) through the lens of metric learning. Standard MHA implicitly learns a static, head-wise Euclidean similarity corresponding to the diagonal blocks of a unified cross-head metric matrix, discarding all off-diagonal interactions across heads. DAMCHA addresses this limitation via two key innovations. First, it learns the full cross-head metric matrix, inducing a Mahalanobis-like similarity that explicitly captures inter-head interactions beyond the restricted block-diagonal structure of MHA. Second, it parameterizes the metric matrix as an input-dependent function, enabling the attention geometry to dynamically adapt to the intrinsic manifold structure of the data rather than remaining fixed after training. We further introduce principled regularization strategies, most notably stack-wise parameter sharing, to ensure computational efficiency and stable optimization. DAMCHA serves as a drop-in replacement for MHA and its variants in various Transformer architectures, delivering superior expressive power and learning performance with comparable or reduced computational overhead. Extensive experiments demonstrate that DAMCHA-based Transformers consistently outperform competing baselines across a range of benchmark tasks. Code is available at https://github.com/erwinmsmith/DAMCHA.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly state DAMCHA's two core innovations:
    learning the full cross-head metric matrix and parameterizing it as an input-dependent function.
    These claims are directly supported by the theoretical proofs, ablation studies, and empirical
    experiments across image generation, text generation, language modeling, and classification
    provided in the paper.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: DAMCHA introduces a learnable metric generator $f_\theta$ shared across
    all layers, which brings a new hyperparameter --- the capacity (depth) of $f_\theta$ --- that may
    require task-specific tuning, as performance improves consistently with deeper generators across
    all evaluated datasets. Additionally, the stack-wise parameter sharing constrains all layers to
    reuse the same family of metric transformations, which may limit layer-specific specialization
    in very deep or highly heterogeneous architectures. These trade-offs are discussed in the
    ablation study.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The strict expressiveness result
    ($\mathcal{S}_{\mathrm{MHA}} \subsetneq \mathcal{S}_{\mathrm{DAMCHA}}$) and the dynamic
    approximation advantage theorem are both proved in full in the appendix. All assumptions are
    explicitly stated prior to each result. The expressiveness proof proceeds via explicit
    construction for containment and a rank-based counterexample for strictness.

\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: All key hyperparameters are reported for each experimental setting,
    including model architecture (number of layers, heads, model and head dimensions), optimizer
    (Adam), learning rates, batch sizes, training steps or epochs, and evaluation metrics.
    Hardware and software configurations are documented in the appendix. An anonymous code
    repository is linked in the introduction.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: An anonymized code repository is provided and linked in the introduction.
    All datasets used are publicly available standard benchmarks, with references and URLs provided
    in the main text and footnotes.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Training details including architecture configuration, optimizer type,
    learning rates, batch sizes, number of training steps or epochs, and evaluation metrics are
    reported for all experimental settings in the main text. Ablation configurations and synthetic
    task settings are detailed in the ablation study and the appendix respectively.

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Error bars are reported in the synthetic regression and classification
    experiments in the appendix. However, the main generation and language modeling results do not
    include error bars, as running multiple full training runs across all methods and datasets on a
    single GPU would be computationally prohibitive given the hardware constraints described in the
    appendix.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The appendix documents the full hardware and software configuration
    (NVIDIA RTX~3090 with 24\,GB VRAM, 12\,vCPU Intel Xeon Platinum 8255C @ 2.50\,GHz,
    Ubuntu~22.04, Python~3.12, PyTorch~2.7.0, CUDA~12.8) and provides approximate wall-clock
    training times for each experimental setting. Per-method memory usage, GFLOPs, and latency
    are also reported in the efficiency comparison table.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: This paper proposes a general-purpose attention mechanism for Transformer
    architectures. It does not involve human subjects, sensitive data collection, or applications
    with direct negative societal impact. All datasets used are standard publicly available
    benchmarks. The work conforms fully with the NeurIPS Code of Ethics.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper presents foundational research on attention mechanisms.
    The proposed method improves general-purpose representation learning and does not introduce
    new capabilities with a direct path to negative applications beyond those already associated
    with standard Transformer models. The societal impacts are consistent with those of general
    machine learning research, as noted in the Impact Statement.

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper proposes an attention mechanism and does not release a large
    pretrained model or scraped dataset. All experiments use standard publicly available benchmarks.
    No high-risk model release is involved, and no specific safeguards are required.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All datasets and baseline methods are properly cited with their original
    publications. Dataset URLs are provided in footnotes where applicable. All baseline methods
    (THA, DCMHA, ColMHA, MoA, MMA) are cited with their original papers. The GPT-2 and ViT
    architectures are used in standard publicly available configurations.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: The DAMCHA attention mechanism is fully described in the method section,
    covering the cross-head metric matrix formulation, adaptive learning procedure, attention
    computation, and the stack-wise sharing mechanism. The end-to-end data flow is further
    illustrated in the appendix. The anonymous code repository contains all training scripts
    and model configurations.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve any crowdsourcing or research with human
    subjects. All experiments are conducted on standard machine learning benchmarks using
    automated evaluation metrics.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: This paper does not involve any research with human subjects.
    No IRB approval is required.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research?
    \item[] Answer: \answerNA{}
    \item[] Justification: LLMs are not used as a core methodological component in this research.
    DAMCHA is evaluated on GPT-2-scale language models as a drop-in attention replacement,
    but the core contribution is the proposed attention mechanism itself. Any use of LLMs was
    limited to writing assistance and does not impact the core methodology, scientific rigor,
    or originality of the research.

\end{enumerate}
